You Get What You Chat: Using Conversations to Personalize Search-based Recommendations

Prior work on personalized recommendations has focused on exploiting explicit signals from user-specific queries, clicks, likes, and ratings. This paper investigates tapping into a different source of implicit signals of interests and tastes: online chats between users. The paper develops an expressive model and effective methods for personalizing search-based entity recommendations. User models derived from chats augment different methods for re-ranking entity answers for medium-grained queries. The paper presents specific techniques to enhance the user models by capturing domain-specific vocabularies and by entity-based expansion. Experiments are based on a collection of online chats from a controlled user study covering three domains: books, travel, food. We evaluate different configurations and compare chat-based user models against concise user profiles from questionnaires. Overall, these two variants perform on par in terms of NCDG@20, but each has advantages in certain domains.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#
# $Id: 
#

.SUFFIXES:
.SUFFIXES: .ps .dvi .tex

TEXINPUTS := .:${TEXINPUTS}
BIBINPUTS := .:${TEXINPUTS}

#all: eps dvi ps pdf # res
all: pdf
eps: fig obj

PAPER=main

LATEX=pdflatex

ps:  $(PAPER).ps

pdf: $(PAPER).pdf
dvi: $(PAPER).dvi

obj: $(patsubst %.obj, %.eps, $(wildcard *.obj))
fig: $(patsubst %.fig, %.eps, $(wildcard *.fig))

res:
	make -C results
	make -C figs

clean:
	$(RM) *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

distclean: clean
	$(RM) $(patsubst %.fig, %.eps, $(wildcard *.fig))
	$(RM) $(patsubst %.obj, %.eps, $(wildcard *.obj))

%.pdf: $(wildcard *.tex) $(wildcard *.bib)
	$(LATEX) $*
	bibtex $*
	$(LATEX) $*
	if [ -e $*.toc ] ; then $(LATEX) $* ; fi
	if [ -e $*.bbl ] ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi

%.ps: %.dvi
	dvips -Ppdf -G0 -tletter -o $@ $<
%.ps.gz: %.ps
	gzip -v9 $<

%.eps: %.obj
	tgif -print -eps $*

%.eps: %.fig
	fig2dev -L eps $< $@

